DeepSemanticHPPC: Hypothesis-based Planning over Uncertain Semantic Point Clouds

Planning in unstructured environments is challenging -- it relies on sensing, perception, scene reconstruction, and reasoning about various uncertainties. We propose DeepSemanticHPPC, a novel uncertainty-aware hypothesis-based planner for unstructured environments. Our algorithmic pipeline consists of: a deep Bayesian neural network which segments surfaces with uncertainty estimates; a flexible point cloud scene representation; a next-best-view planner which minimizes the uncertainty of scene semantics using sparse visual measurements; and a hypothesis-based path planner that proposes multiple kinematically feasible paths with evolving safety confidences given next-best-view measurements. Our pipeline iteratively decreases semantic uncertainty along planned paths, filtering out unsafe paths with high confidence. We show that our framework plans safe paths in real-world environments where existing path planners typically fail.

==> sections/methods.tex <==
\subsection{Pipeline}

Figure \ref{fig:Pipeline} show the proposed NBV planner. First, a detector extracts semantic segmentations along with uncertainties from a new image measurement. The information is used to project an uncertain semantic point cloud, which is then fused with the previous point cloud scene model. The fused point cloud is then the input into a neural network which calculates a utility function, which is used for a reinforcement learning agent to plan the NBV. The robot then takes a new image at the NBV and the pipeline is repeated until termination criteria is met. An example would be observing an object such as a person in a forest. At first there is high uncertainty around the detection which could potentially be a person or a wooden log. The detection of people has high relevance to a task so the NBV plans a new measurement close to the uncertain person detection. The new measurement is taken and fused into the existing scene which refines the previous person segmentation and reduces uncertainty.

\begin{figure*}
\begin{center}
\includegraphics[width=1\linewidth]{figs/Pipeline2.png}
\end{center}
   \caption{Pipeline of the NBV planner and scene reconstruction. The detector  extracts information from a new image measurement, which is fused together with the previous scene representation, which is then used for the input to the NBV planner. Another image is taken and the process is repeated.}
\label{fig:Pipeline}
\end{figure*}

%\begin{figure}[]
%   \centering \includegraphics[width=1\linewidth]{figs/Pipeline.png} \caption{Pipeline of the NBV planner and scene reconstruction. The detector (left block) extracts information from raw images, which are fused together with the previous scene representation (middle block) and used for the input to the NBV planner (right block). Another image is taken and the process is repeated. In the lower right is an example where an initial measurement of an object (trashcan) has high uncertainty, but after taking the NBV measurement, the uncertainty is reduced.} \label{fig:Pipeline}
%\end{figure}

\subsection{Pixelwise Uncertainty and Point Cloud Fusion}

Each image is composed of a set of $n_{p}$ pixels $P = \{p^{1},...p^{k},...p^{n_{p}}\}$ where $p^{k}$ is an individual pixel. Semantic segmentations are extracted from camera frames for fusion, using state of the art neural networks \cite{DeeplabV3}. To get bayesian uncertainties from the semantic segmentations, the dropout approximation method for BNNs is used \cite{Gal2016Dropout} during runtime. During runtime, multiple stochastic runs of the network with dropout are performed and the statistics of the results are analyzed to calculate the segmentation uncertainties. These pixelwise uncertainties are calculated as:

$$
\sigma_{c_{i}} = \textrm{Var}(p_{c_{i}}\|_1^{n_{d}})
\eqno{(2)}
$$
where $\sigma_{c_{i}}$ is the uncertainty for class $i = [1,...n_{c}]$ where $n_c$ is the number of semantic classes. $p_{c_{i}}$ is the output of the probability vector for class $i$ and $n_{d}$ is the number of stochastic dropout runs. Refer to \cite{KendallUncert} for a more detailed description of calculation of BNN uncertainties. Figure \ref{fig:BNNUncert} shows the result of the BNN network on the \textcolor{red}{ref} dataset. The uncertainties tend to be highest around edges and boundaries between different semantic classes.

\begin{figure}[]
   \centering \includegraphics[width=0.8\linewidth]{figs/BNNUncert.png} \caption{Results from the BNN dropout method. \textbf{Top}: The original image. \textbf{Middle}: Semantic segmentations. \textbf{Bottom}: The uncertainties from the BNN. Lighter color represents higher uncertainties. The high uncertainties are generally concentrated edges and boundaries between surfaces.} \label{fig:BNNUncert}
\end{figure}

%Depth maps are simultaneously acquired using stereo vision with Semi-Global Block Matching (SGBM) \cite{SGBM}, which is a standard block matching stereo vision algorithm. The depth maps and camera parameters are used to project the image pixels into a 3D point cloud along semantic class labels and the associated uncertainties. Positional uncertainties based on the stereo algorithm are found with the following standard equations \cite{PTGrey}:
%
%$$
%\sigma_{x}, \sigma_{y} = \frac{p*z}{f}
%\eqno{(2)}
%$$
%
%$$
%\sigma_{z} = \frac{-z^{2}}{f*b}*d
%\eqno{(2)}
%$$
%where $\{\sigma_{x}, \sigma_{y}, \sigma_{z}\}$ are uncertainties in the projected $\{x,y,z\}$ coordinates. For the image coordinate system: $x-\textrm{axis}$ is going to the right, $y-\textrm{axis}$ is going up, and $z-\textrm{axis}$ is going into the image. $p$ is the calibration error for the camera, $f$ is the focal length, $z$ is the predicted depth, $b$ is the camera baseline, and $d$ is the disparity error based on the stereo algorithm.

Each $p^{k}$ is associated with: (1) $c_{p^{k},max}$ and $\sigma_{p^{k},c_{max}}$ which are the class with highest average probability and the associated uncertainty, which will be denoted as $c_{k}$ and $\sigma_{c_{k}}$ from henceforth. (2) $\{x_{k}, y_{k}, z_{k}\}$ which are projected 3D positions using the camera parameters.%(2) $\{x_{k}, y_{k}, z_{k}\}$ and $\{\sigma_{x_{k}}, \sigma_{y_{k}}, \sigma_{z_{k}}\}$, which are the 3D positions along with their respective uncertainties.

For point cloud fusion of multiple images, points are fused with the result from the best linear unbiased estimator (BLUE) \cite{DWFusion}. Given two noisy measurements of a variable $X \sim \mathcal{N}(\mu,\,\sigma^{2})$, the combined measurement is:

$$
\bar{X} = \frac{\sigma_{1}^{2}}{\sigma_{1}^{2} + \sigma_{1}^{2}}*\mu_{1} + \frac{\sigma_{2}^{2}}{\sigma_{1}^{2} + \sigma_{1}^{2}}*\mu_{2}
\eqno{(2)}
$$

$$
\sigma_{\bar{X}}^{2} = \bigg(\frac{1}{\sigma_{1}^{2}} + \frac{1}{\sigma_{2}^{2}}\bigg)^{-1}
\eqno{(2)}
$$
where the two measurements are $\{X_1 \sim \mathcal{N}(\mu_{1},\,\sigma_{1}^{2}), X_2 \sim \mathcal{N}(\mu_{2},\,\sigma_{2}^{2})\}$ and $\bar{X}$ and $\sigma_{\bar{X}}^{2}$ are the combined measurement and its noise respectively. The combined measurement is intuitively weighted more towards the measurement with lower uncertainty. 

Points are fused if they are deemed redundant. If a combined point would be inside the overlap of the covariance of two current points, the current points are considered redundant. The Mahalanobis distance is used as a threshold to determine if a combined point is within the covariance of two current points \cite{MergeOverlap}.

\subsection{Frontier Definition and Discovery}

In this paper the intuitive definition of a frontier boundary is a boundary of interest for exploration or refinement. Formally, a frontier boundary is defined as (1) the transition from dense to sparse points (density boundary) or (2) the boundary between two different semantic classes (semantic boundary).  The combination of the two boundaries makes it straightforward to encode exploration and task-dependent refinement into a utility function. The use of the density boundary is similar to \cite{SEE}, which uses a density representation to identify the frontier as a more flexible alternative to traditional grid based methods. The density boundary is intuitively defined as the intersection between dense and sparse points. It makes the assumption that explored space is densely populated, and unexplored space is sparse. The density boundary is used to encode exploration of unexplored space in the utility function. The semantic boundary represents the intersection between two different classes. Figure \ref{fig:BNNUncert} shows that boundaries between classes tend to have the highest uncertainty. These semantic boundaries encode refinement of explored space for task-dependent NBV planning.

To find density boundary points a method similar to DBSCAN is used \cite{DBSCAN}. A neighborhood with radius $r_{den}$ is defined around each point. Points with greater than $k_{min}$ other points within their neighborhood are classified as core points or dense points. Points with less than $k_{max}$ points within their neighborhood are classified as sparse points. All other points are classified as density boundary points. Figure \ref{fig:DenFront} shows point labels from the boundary detection algorithm. Semantic boundary points are found by defining a neighborhood with radius $r_{sem}$ around each point. Points with greater than 1 class within their neighborhood are labeled as semantic boundary points. Figure \ref{fig:SemFront} shows labeled semantic points with boundary points in teal.

\begin{figure}[]
   \centering \includegraphics[width=0.8\linewidth]{figs/DenFront.png} \caption{Discovery of density frontier points. Corepoints are shown in blue, density frontier points are shown in green, and sparse points are shown in red. A neighborhood of radius $r_{den}$ is defined around each point. Points with greater than $k_{min}$ points inside their neighborhood are labeled core points, points with less than $k_{max}$ points within their neighborhood are labeled sparse points, and the remaining points are density frontier points.} \label{fig:DenFront}
\end{figure}

\begin{figure}[]
   \centering \includegraphics[width=0.8\linewidth]{figs/SemFront.png} \caption{Discovery of semantic frontier points. Points in orange belong to one semantic class and points in purple belong to another semantic class. Points in teal are the semantic frontier points. A neighborhood of radius $r_{sem}$ is defined around each point, and points with greater than one class inside their neighborhood are considered semantic frontier points.} \label{fig:SemFront}
\end{figure}

\subsection{Utility Function Definition and Learning}

The utility function is designed to weight exploration of unknown space and refinement of previously explored space, depending on the task. Informally, the utility function seeks to reduce uncertainty at the boundaries (density or semantic) which are relevant to the task. Formally, the utility function is defined as:

$$
E = \sum_{i=1}^{n_{c}+1} w_{i}*\sigma_{i,avg}
\eqno{(2)}
$$

$$
U = E_{final} - E_{initial}
\eqno{(2)}
$$
where $U$ is the target utility function, $n_{c}$ is the number of classes, $w$ is a weighting term, and $\sigma_{i,avg}$ is an uncertainty measure for each boundary. $E_{initial}$ is the sum of weighted average boundary uncertainties in the initial point cloud, and $E_{final}$ is the sum of weighted average boundary uncertainties in the final fused point cloud after fusing a new image. $i\|_{1}^{n_{c}+1}$ because there are $n_{c}$ semantic classes which make up $n_{c}$ semantic frontier boundaries and also one additional boundary type which is the density frontier boundary. To calculate $\sigma_{i,avg}$ for each boundary type, a volume is defined around each boundary type and the uncertainties inside that volume are averaged. The points inside the defined volume are found by finding all points within a radius $r_{v}$ of the desired boundary points. Then the average uncertainties for each boundary type are weighted by $w_{i}$ to account for the task-dependent NBV planning. For tasks that need more exploration (for example, mapping an environment with no prior knowledge) the utility is weighted towards the uncertainty around density boundary points, for tasks that need refinement of specific semantic classes (for example, detecting the boundary between navigable surfaces, such as grass, and non-navigable surfaces, such as mud) the utility is weighted towards the uncertainty around those specific semantic classes, hence Semantic Next-Best-View. 

The utility prediction network is a mapping from an input point cloud, and a pose of a potential next camera measurement to a utility function with hand defined weights. The initial point cloud is transformed by parameters of the next view to encode the pose the next measurement will be taken at. The input to the network is an array of 3D points $\{x_{k}, y_{k}, z_{k}\}$ along with class labels and uncertainties, $c_{k}$ and $\sigma_{c_{k}}$ respectively. PointNet is used as the basis for the network \cite{PointNet}.

Generating training samples is done by creating pairs which consist of (1) initial point clouds transformed by the next camera pose and (2) the task-dependent utility function. Sets of initial images close in distance and oriented towards a single point (to simulate an initial reconstruction) are first fused using the methods described in section 3.2. Then next measurement images are sampled close to the initial point cloud to simulate the next view and fused into the initial measurement. The utility function is then calculated using the initial and final fused point clouds.

\subsection{Reinforcement Learning}
\textcolor{teal}{Theres no hope}

==> sections/related.tex <==

\subsection{Semantic 3D Reconstruction}

Recovering 3D structure of a scene from camera images is a well studied problem. The traditional pipeline uses Structure from Motion (SfM) and Multiview Stereo (MVS) algorithms to recover both camera parameters and depth clouds from each image, using feature matching, camera parameter geometry, and techniques such as bundle adjustment and image registration \cite{COLMAP}, \cite{SnavelyPhotoTour}, \cite{SurveySfM}. The depth clouds are then fused together into a scene representation. Generally, these methods do not reconstruct scenes with any semantic information, nor do they use semantic information to help with reconstructing the scene. Semantic Structure from Motion (SSfM) extends the traditional SfM pipeline to also account for semantic labels for object detections \cite{SSfM}, \cite{SSfMRegions}. By solving for camera and object parameters (pose) simultaneously, SSfM is able to recover scene geometry with fewer images while also discovering semantic scene information. In iterative SfM reconstruction methods, the NBV is generally chosen with a heuristic, such as the image with the most triangulated points. It is important to note that in SfM, all the images have already been collected at the start. No new data is acquired.

As the motivation for this paper is using an autonomous robotic agent to reconstruct an environment, the camera parameters are assumed to be known. The ECCV semantic reconstruction challenge \cite{ECCV2018} provides a synthetic garden dataset with ground truth segmentations and depth. The challenge is to reconstruct the scene into a semantic mesh given the camera parameters, using as many images as desired. The participants generally extracted semantic and depth information with well known vision techniques (neural nets, stereo depth, etc.) and refined fused point clouds before generating a mesh. This paper considers the additional challenges of formalizing uncertainty, and finding the NBV, and reconstruction with just a few images.

\subsection{Next Best View}

A popular approach to estimating the NBV uses an information gain (IG) calculated from a voxel based scene representation \cite{CompVIG}, \cite{DaudNBV}, \cite{LearntoScore}. Each voxel has a probability of being occupied and the uncertainty is calculated as the entropy in the voxel. The NBV is chosen by raycasting from potential viewpoints and calculating objectives, such as minimizing entropy or viewing occluded objects (by assigning higher weights to unseen voxels next to seen and occupied voxels). These voxel based representations are generally good for single object reconstruction, but scale poorly to large scenes, due to computational complexity of high resolution voxels. Surface representations scale better to large scenes but require fine tuning of unintuitive parameters \cite{SEE}, \cite{GPUAV}.

There community has developed several frontier based NBV approaches \cite{DynamicFrontier}, \cite{FrontierSwarm}. Frontiers represent the boundary between explored and unexplored space. These approaches generally do not take advantage of semantic scene information and designate the NBV as the closest frontier, or the frontier viewing frustum that contains the most unseen voxels \cite{HorizonNBV}. Work has been done to balance pure exploration with refinement of the scene \cite{NBVRefine}, but this approach also does not account for semantic information.

The Surface Edge Explorer (SEE) \cite{SEE}, uses a frontier based approach for finding the NBV and a density based point cloud representation of the scene. Here, the frontier is defined as the boundary between dense and sparse points. The density based frontier discovery allows for a flexible scene representation and an intuitive definition of where the NBV could be. The SEE was tested on single object detection, without the inclusion of semantic information.

There has been work on NBV planning for object detection and pose estimation \cite{6DOFNBV}. This approach explores single-shot 6D object pose with multiple objects in the scene and plans the NBV based on uncertainty reduction. The paper is not focused on scene reconstruction, but only object bounding box generation.

\subsection{Treatment of Uncertainty}

The community has developed methods to deal with fusion of uncertain and redundant point clouds \cite{MergeOverlap}, \cite{3DRGBDFuse}. These methods experiment with depth from sensors such as the Microsoft Kinect and add pointwise uncertainty to the point clouds based on the camera parameters. Points with overlapping covariances are considered redundant have both positions and uncertainties fused with more weight assigned to more certain points. These works provide a principled way to deal with depth uncertainty but do not address pointwise semantic uncertainty. 

Many approaches to formally address uncertainty in neural network outputs, such as pixelwise segmentation, have been developed. One approach is to use calibrated probabilities which leverages temperature scaling to calibrate the predictions of networks \cite{GuoCalib}. This approach does not provide a formal mathematical treatment of the uncertainty. A more formal treatment of uncertainty uses Bayesian Neural Networks (BNNs) which perform posterior inference over the weights of the network nodes \cite{SimpleNNMDL}, \cite{PracticalVI}. BNNs are traditionally computationally expensive because variational inference is required for posterior inference. To speed up computational speed to make online implementations feasible, the dropout method has been developed to perform approximate inference for BNNs \cite{Gal2016Dropout}, \cite{KendallUncert}, \cite{BNNDisease}. Essentially, during online prediction, multiple stochastic runs of the network are performed with dropout and the statistics of the results are analyzed to produce mathematically principled estimates of network uncertainty. To the best of the authors knowledge, formal treatment of pointwise semantic uncertainty in scene reconstruction and NBV planning has not been previously addressed in the vision community.

\subsection{Reinforcement Learning}
\textcolor{cyan}{LOL idk}
\textcolor{red}{ref}

The work closest to this paper uses a neural network to learn a utility function for finding the NBV \cite{LearntoScore}, with a voxel based representation for the scene. The utility function is calculated based on the reduction in uncertainty over the entire scene. However, the uncertainty is treated as a heuristic and assumed to be monotonically decreasing with more image measurements and the utility function is not task based. The NBV is also limited to grid locations surrounding the camera. In this paper, a formal treatment of pixelwise uncertainty is developed and a task-dependent utility function is used. In addition, a more flexible point cloud representation is used as the input to the neural network. This paper also has no grid-based restriction on the possible NBV location.
